DistiLLM: Towards Streamlined Distillation for Large Language Models

Knowledge distillation (KD) is widely used for compressing a teacher model to a smaller student model, reducing its inference cost and memory footprint while preserving model capabilities. However, current KD methods for auto-regressive sequence models (e.g., large language models) suffer from missing a standardized objective function. Moreover, the recent use of student-generated outputs to address training-inference mismatches has significantly escalated computational costs. To tackle these issues, we introduce DistiLLM, a more effective and efficient KD framework for auto-regressive language models. DistiLLM comprises two components: (1) a novel skew Kullback-Leibler divergence loss, where we unveil and leverage its theoretical properties, and (2) an adaptive off-policy approach designed to enhance the efficiency in utilizing student-generated outputs. Extensive experiments, including instruction-following tasks, demonstrate the effectiveness of DistiLLM in building high-performing student models while achieving up to 4.3$\times$ speedup compared to recent KD methods.

==> qualitative/self_inst.tex <==
\newpage
\begin{table*}[t]
\centering
\vspace{-10pt}
\caption{Self-Instruct.}
\vspace{5pt}
% \renewcommand{\arraystretch}{1.1}
\resizebox{1.0\textwidth}{!}{
\addtolength{\tabcolsep}{2.5pt}
\begin{tabular}{m{3cm}|m{20cm}}
\toprule[0.1em]
        \multicolumn{2}{c}{\textbf{\textit{Case \# 1}}} \\ \midrule[0.1em]
        Instruction &  \\ \midrule
        Input &  \\ \midrule \midrule
        SFT &  \\
        \midrule
        KD &  \\
        \midrule
        SeqKD &  \\
        \midrule
        ImitKD &  \\
        \midrule
        MiniLLM &  \\
        \midrule
        GKD &  \\
        \midrule
        \alg &  \\ \midrule[0.1em]
        \multicolumn{2}{c}{\textbf{\textit{Case \# 2}}} \\ \midrule[0.1em]
        Instruction &  \\ \midrule
        Input &  \\ \midrule \midrule
        SFT &  \\
        \midrule
        KD &  \\
        \midrule
        SeqKD &  \\
        \midrule
        ImitKD &  \\
        \midrule
        MiniLLM &  \\
        \midrule
        GKD &  \\
        \midrule
        \alg &  \\ \midrule[0.1em]
        \multicolumn{2}{c}{\textbf{\textit{Case \# 3}}} \\ \midrule[0.1em]
        Instruction &  \\ \midrule
        Input &  \\ \midrule \midrule
        SFT &  \\
        \midrule
        KD &  \\
        \midrule
        SeqKD &  \\
        \midrule
        ImitKD &  \\
        \midrule
        MiniLLM &  \\
        \midrule
        GKD &  \\
        \midrule
        \alg &  \\
\bottomrule[0.1em]
\end{tabular}
}\label{qualitative:self}
\end{table*}

==> src/fig_ablation.tex <==
\begin{figure*}[t]
    \hspace*{\fill}
    \begin{subfigure}[b]{0.24\textwidth} % 0.4 % 0.23
    \centering
    \includegraphics[width=\linewidth]{example-image}
    \caption{MRPC} \label{fig:distillm_alpha}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth} % 0.4 % 0.23
    \centering
    \includegraphics[width=\linewidth]{example-image}
    \caption{RTE} \label{fig:fkl_rkl}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth} % 0.4 % 0.23
    \centering
    \includegraphics[width=\linewidth]{example-image}
    \caption{SST-2} \label{fig:variance}
    \end{subfigure} 
    \hfill
    \begin{subfigure}[b]{0.24\textwidth} % 0.4 % 0.23
    \centering
    \includegraphics[width=\linewidth]{example-image}
    \caption{Supp RTE} \label{fig:time}
    \end{subfigure}
    \caption{We compare the performance for different layer mapping functions and distillation objectives in (a)-(c). The distillations of the last layer, uniform layer mapping, self-attention, and IR are denoted by L, U, S, and R, respectively. The blue\,(Enc.) and orange\,(Dec.) bar denote the application of ILD to the decoder network only and to both encoder and decoder network, respectively. We also denote ILD with CA and CR as the green and brown bars in (a)-(c), respectively. (d)-(e) are results for using ST for TTs of MRPC and RTE. We only distill self-attention of the last layer of the decoder when using ILD with ST and CR}\label{fig:appx_t5}
\end{figure*}

==> src/fig_l2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/fig_generalizability.pdf}
    \vspace{-17.5pt}
    \caption{Distribution of differences between EMA and instant divergence values. \textcolor{red}{As shown in Theorem~\ref{method:thm}, both SKL and SRKL have reduced L2 norm value as $\alpha$ increases. For normalized values by related EMA values, SKL and SRKL with $\alpha=0.1$ only shows the effectiveness which support the results in Sec.~\ref{sec:exp}}.}
    \label{fig:fig_l2}
    \vspace{-10pt}
\end{figure}
